The Borel Cohomology of Free Iterated Loop Spaces

We compute the $\rm{SO}(n+1)$-equivariant mod $2$ Borel cohomology of the free iterated loop space $Z^{S^n}$ when $Z$ is a mod $2$ generalized Eilenberg Mac Lane space. When $n=1$, this recovers B\"okstedt and Ottosen's computation for the free loop space. The highlight of our computation is a construction of cohomology classes using an $\mathrm{O}(n)$-equivariant evaluation map and a pushforward map.

==> mymacros.tex <==
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\SP}{\mathbb{S}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\FF}{\mathbb{F}}
\renewcommand{\AA}{\mathbb{A}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\ts}{\textsuperscript}
\newcommand{\mf}{\mathfrak}
\newcommand{\cc}{\mf{c}}
\newcommand{\mg}{\mf{g}}
\newcommand{\ma}{\mf{a}}
\newcommand{\mh}{\mf{h}}
\newcommand{\mn}{\mf{n}}
\newcommand{\mc}{\mf{c}}
\newcommand{\ul}{\underline}
\newcommand{\mz}{\mf{z}}
\newcommand{\me}{\mf{e}}
\newcommand{\mff}{\mf{f}}
\newcommand{\mm}{\mf{m}}
\newcommand{\mt}{\mf{t}}
\newcommand{\pp}{\mf{p}}
\newcommand{\qq}{\mf{q}}
\newcommand{\gl}{\mf{gl}}
\newcommand{\msl}{\mf{sl}}
\newcommand{\so}{\mf{so}}
\newcommand{\mfu}{\mf{u}}
\newcommand{\su}{\mf{su}}
\newcommand{\GEM}{\mathrm{GEM}}
\newcommand{\ft}{\mathrm{ft}}
\newcommand{\gr}{\mathrm{gr}}
\newcommand{\fin}{\mathrm{fin}}

\newcommand{\msp}{\mf{sp}}
\renewcommand{\aa}{\mf{a}}
\newcommand{\bb}{\mf{b}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\lb}{\langle}
\newcommand{\rb}{\rangle}
\newcommand{\ff}{\mf{f}}
\newcommand{\ee}{\epsilon}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}

\newcommand{\pushout}{\arrow[ul, phantom, "\ulcorner", very near start]}
\newcommand{\pullback}{\arrow[dr, phantom, "\lrcorner", very near start]}

\newcommand{\simp}[1]{#1^{\Delta^{op}}}

\newcommand{\arrowtcupp}[2]{\arrow[bend left=50, ""{name=U, below,inner sep=1}]{#1}\arrow[Rightarrow,from=U,to=MU,"#2"]}
\newcommand{\arrowtclow}[2]{\arrow[bend right=50, ""{name=L,inner sep=1}]{#1}\arrow[Rightarrow,from=LM,to=L]{}[]{#2}} % if you want to change some parameter of the label.
\newcommand{\arrowtcmid}[2]{\arrow[""{name=MU,inner sep=1},""{name=LM,below,inner sep=1}]{#1}[pos=.1]{#2}}
\newcommand{\dummy}{\textcolor{white}{\bullet}}


%for adjunction
\newcommand{\adjunction}[4]{
	#1\hspace{2pt}\colon #2	\leftrightharpoons #3 \hspace{2pt}\colon #4
}


%Math operators
\newcommand{\gem}{\mathop{\rm gem}\nolimits}
\newcommand{\Set}{\mathop{\rm Set}\nolimits}
\newcommand{\Spaces}{\mathop{\rm Space}\nolimits}
\newcommand{\Ind}{\mathop{\rm Ind}\nolimits}
\newcommand{\Sind}{\mathop{\rm Sind}\nolimits}
\newcommand{\Ext}{\mathop{\rm Ext}\nolimits}
\newcommand{\sd}{\mathop{\rm sd}\nolimits}
\newcommand{\Ex}{\mathop{\rm Ex}\nolimits}
\newcommand{\Out}{\mathop{\rm Out}\nolimits}
\newcommand{\Cyl}{\mathop{\rm Cyl}\nolimits}
\newcommand{\Path}{\mathop{\rm Path}\nolimits}
\newcommand{\Ch}{\mathop{\rm Ch}\nolimits}
\newcommand{\SSet}{\mathop{\rm \Set^{\Delta^{op}}}\nolimits}
\newcommand{\Sq}{\mathop{\rm Sq}\nolimits}
\newcommand{\Free}{\mathop{\rm Free}\nolimits}
\newcommand{\Maps}{\mathop{\rm Maps}\nolimits}
\newcommand{\LMaps}{\mathop{\rm LMaps}\nolimits}
\newcommand{\RMaps}{\mathop{\rm RMaps}\nolimits}
\newcommand{\MU}{\mathop{\rm MU}\nolimits}
\newcommand{\MSU}{\mathop{\rm MSU}\nolimits}
\newcommand{\MSp}{\mathop{\rm MSp}\nolimits}
\newcommand{\MSO}{\mathop{\rm MSO}\nolimits}
\newcommand{\MO}{\mathop{\rm MO}\nolimits}
\newcommand{\BU}{\mathop{\rm BU}\nolimits}
\newcommand{\BSU}{\mathop{\rm BSU}\nolimits}
\newcommand{\BSp}{\mathop{\rm BSp}\nolimits}
\newcommand{\BSO}{\mathop{\rm BSO}\nolimits}
\newcommand{\BO}{\mathop{\rm BO}\nolimits}
\newcommand{\Tor}{\mathop{\rm Tor}\nolimits}
\newcommand{\Cotor}{\mathop{\rm Cotor}\nolimits}
\newcommand{\imag}{\mathop{\rm Im}\nolimits}
\newcommand{\real}{\mathop{\rm Re}\nolimits}
\newcommand{\Cat}{\mathop{\rm Cat}\nolimits}
\newcommand{\Fld}{\mathop{\rm Fld}\nolimits}
\newcommand{\Frac}{\mathop{\rm Frac}\nolimits}
\newcommand{\Dom}{\mathop{\rm Dom}\nolimits}
\newcommand{\Hotc}{\mathop{\rm Hotc}\nolimits}
\newcommand{\Top}{\mathop{\rm Top}\nolimits}
\newcommand{\Ring}{\mathop{\rm Ring}\nolimits}
\newcommand{\CRing}{\mathop{\rm CRing}\nolimits}
\newcommand{\CGHaus}{\mathop{\rm CGHaus}\nolimits}
\newcommand{\Alg}{\mathop{\rm Alg}\nolimits}
\newcommand{\Bool}{\mathop{\rm Bool}\nolimits}
\newcommand{\hTop}{\mathop{\rm hTop}\nolimits}
\newcommand{\Nat}{\mathop{\rm Nat}\nolimits}
\newcommand{\Rel}{\mathop{\rm Rel}\nolimits}
\newcommand{\Mod}{\mathop{\rm Mod}\nolimits}
\newcommand{\Space}{\mathop{\rm Space}\nolimits}
\newcommand{\Vect}{\mathop{\rm Vect}\nolimits}
\newcommand{\FinVect}{\mathop{\rm FinVect}\nolimits}
\newcommand{\Matr}{\mathop{\rm Matr}\nolimits}
\newcommand{\Ab}{\mathop{\rm Ab}\nolimits}
\newcommand{\Gr}{\mathop{\rm Gr}\nolimits}
\newcommand{\Grp}{\mathop{\rm Grp}\nolimits}
\newcommand{\Hol}{\mathop{\rm Hol}\nolimits}
\newcommand{\Grpd}{\mathop{\rm Grpd}\nolimits}
\newcommand{\Mon}{\mathop{\rm Mon}\nolimits}
\newcommand{\FinSet}{\mathop{\rm FinSet}\nolimits}
\newcommand{\Sch}{\mathop{\rm Sch}\nolimits}
\newcommand{\AffSch}{\mathop{\rm AffSch}\nolimits}
\newcommand{\Idem}{\mathop{\rm Idem}\nolimits}
\newcommand{\SIdem}{\mathop{\rm SIdem}\nolimits}
\newcommand{\Aut}{\mathop{\rm Aut}\nolimits}
\newcommand{\Ord}{\mathop{\rm Ord}\nolimits}
\newcommand{\coker}{\mathop{\rm coker}\nolimits}
\newcommand{\ch}{\mathop{\rm char}\nolimits}%characteristic
\newcommand{\Sym}{\mathop{\rm Sym}\nolimits}
\newcommand{\adj}{\mathop{\rm adj}\nolimits}
\newcommand{\dil}{\mathop{\rm dil}\nolimits}
\newcommand{\Cl}{\mathop{\rm Cl}\nolimits}
\newcommand{\Diff}{\mathop{\rm Diff}\nolimits}
\newcommand{\End}{\mathop{\rm End}\nolimits}
\newcommand{\Hom}{\mathop{\rm Hom}\nolimits}% preferred
\newcommand{\Gal}{\mathop{\rm Gal}\nolimits}
\newcommand{\Pos}{\mathop{\rm Pos}\nolimits}
\newcommand{\Ad}{\mathop{\rm Ad}\nolimits}
\newcommand{\GL}{\mathop{\rm GL}\nolimits}
\newcommand{\SL}{\mathop{\rm SL}\nolimits}
\newcommand{\vol}{\mathop{\rm vol}\nolimits}
\newcommand{\reg}{\mathop{\rm reg}\nolimits}
\newcommand{\Or}{\rm O}
\newcommand{\U}{\mathop{\rm U}\nolimits}
\newcommand{\SOr}{\mathop{\rm SO}\nolimits}
\newcommand{\BOr}{\mathop{\rm BO}\nolimits}
\newcommand{\BSOr}{\mathop{\rm BSO}\nolimits}
\newcommand{\SU}{\mathop{\rm SU}\nolimits}
\newcommand{\Spin}{\mathop{\rm Spin}\nolimits}
\newcommand{\Sp}{\mathop{\rm Sp}\nolimits}
\newcommand{\Int}{\mathop{\rm Int}\nolimits}
\newcommand{\im}{\mathop{\rm im}\nolimits}
\newcommand{\dom}{\mathop{\rm dom}\nolimits}
\newcommand{\di}{\mathop{\rm div}\nolimits}
\newcommand{\cod}{\mathop{\rm cod}\nolimits}
\newcommand{\colim}{\mathop{\rm colim}\nolimits}
\newcommand{\ad}{\mathop{\rm ad}\nolimits}
\newcommand{\PSL}{\mathop{\rm PSL}\nolimits}
\newcommand{\PGL}{\mathop{\rm PGL}\nolimits}
\newcommand{\sep}{\mathop{\rm sep}\nolimits}
\newcommand{\MCG}{\mathop{\rm MCG}\nolimits}
\newcommand{\oMCG}{\mathop{\rm MCG^+}\nolimits}
\newcommand{\Spec}{\mathop{\rm Spec}\nolimits}
\newcommand{\rank}{\mathop{\rm rank}\nolimits}
\newcommand{\diverg}{\mathop{\rm div}\nolimits}%Divergence
\newcommand{\disc}{\mathop{\rm disc}\nolimits}
\newcommand{\sign}{\mathop{\rm sign}\nolimits}
\newcommand{\Arf}{\mathop{\rm Arf}\nolimits}
\newcommand{\Pic}{\mathop{\rm Pic}\nolimits}
\newcommand{\Tr}{\mathop{\rm Tr}\nolimits}
\newcommand{\res}{\mathop{\rm res}\nolimits}
\newcommand{\Proj}{\mathop{\rm Proj}\nolimits}
\newcommand{\mult}{\mathop{\rm mult}\nolimits}
\newcommand{\N}{\mathop{\rm N}\nolimits}
\newcommand{\lk}{\mathop{\rm lk}\nolimits}
\newcommand{\Pf}{\mathop{\rm Pf}\nolimits}
\newcommand{\sgn}{\mathop{\rm sgn}\nolimits}
\newcommand{\grad}{\mathop{\rm grad}\nolimits}
\newcommand{\lcm}{\mathop{\rm lcm}\nolimits}
\newcommand{\Ric}{\mathop{\rm Ric}\nolimits}
\newcommand{\Hess}{\mathop{\rm Hess}\nolimits}
\newcommand{\sn}{\mathop{\rm sn}\nolimits}
\newcommand{\cut}{\mathop{\rm cut}\nolimits}
\newcommand{\tr}{\mathop{\rm tr}\nolimits}
\newcommand{\codim}{\mathop{\rm codim}\nolimits}
\newcommand{\ind}{\mathop{\rm index}\nolimits}
\newcommand{\rad}{\mathop{\rm rad}\nolimits}
\newcommand{\Rep}{\mathop{\rm Rep}\nolimits}
\newcommand{\Lie}{\mathop{\rm Lie}\nolimits}
\newcommand{\Der}{\mathop{\rm Der}\nolimits}
\newcommand{\hgt}{\mathop{\rm ht}\nolimits}
\newcommand{\Ider}{\mathop{\rm Ider}\nolimits}
\newcommand{\id}{\mathop{\rm id}\nolimits}
